Pretraining Image Encoders without Reconstruction via Feature Prediction Loss

This work investigates three methods for calculating loss for autoencoder-based pretraining of image encoders: The commonly used reconstruction loss, the more recently introduced deep perceptual similarity loss, and a feature prediction loss proposed here; the latter turning out to be the most efficient choice. Standard auto-encoder pretraining for deep learning tasks is done by comparing the input image and the reconstructed image. Recent work shows that predictions based on embeddings generated by image autoencoders can be improved by training with perceptual loss, i.e., by adding a loss network after the decoding step. So far the autoencoders trained with loss networks implemented an explicit comparison of the original and reconstructed images using the loss network. However, given such a loss network we show that there is no need for the time-consuming task of decoding the entire image. Instead, we propose to decode the features of the loss network, hence the name "feature prediction loss". To evaluate this method we perform experiments on three standard publicly available datasets (LunarLander-v2, STL-10, and SVHN) and compare six different procedures for training image encoders (pixel-wise, perceptual similarity, and feature prediction losses; combined with two variations of image and feature encoding/decoding). The embedding-based prediction results show that encoders trained with feature prediction loss is as good or better than those trained with the other two losses. Additionally, the encoder is significantly faster to train using feature prediction loss in comparison to the other losses. The method implementation used in this work is available online: https://github.com/guspih/Perceptual-Autoencoders

==> acronym.tex <==
\begin{acronym}[Bash]
    % General
    
    % A
    \acro{AI}{Artificial Intelligence}
    \acro{ANN}{Artificial Neural Network}
    
    % C 
    \acro{CNN}{Convolutional Neural Network}
    
    % F
    \acro{FP}{feature prediction}
    
    % M
    \acro{MLP}{Multilayer Perceptron}
    
    % N
    \acro{NC-Net}{Neighbourhood Consensus Network}
    
     % P
    \acro{PW}{pixel-wise}
    \acro{PS}{perceptual similarity}
    
    % R
    \acro{RL}{Reinforcement Learning}
    
   
    
\end{acronym}
